Geo-Graph-Indistinguishability: Location Privacy on Road Networks Based on Differential Privacy

In recent years, concerns about location privacy are increasing with the spread of location-based services (LBSs). Many methods to protect location privacy have been proposed in the past decades. Especially, perturbation methods based on Geo-Indistinguishability (Geo-I), which randomly perturb a true location to a pseudolocation, are getting attention due to its strong privacy guarantee inherited from differential privacy. However, Geo-I is based on the Euclidean plane even though many LBSs are based on road networks (e.g. ride-sharing services). This causes unnecessary noise and thus an insufficient tradeoff between utility and privacy for LBSs on road networks. To address this issue, we propose a new privacy notion, Geo-Graph-Indistinguishability (GG-I), for locations on a road network to achieve a better tradeoff. We propose Graph-Exponential Mechanism (GEM), which satisfies GG-I. Moreover, we formalize the optimization problem to find the optimal GEM in terms of the tradeoff. However, the computational complexity of a naive method to find the optimal solution is prohibitive, so we propose a greedy algorithm to find an approximate solution in an acceptable amount of time. Finally, our experiments show that our proposed mechanism outperforms a Geo-I's mechanism with respect to the tradeoff.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/geogi_old.tex <==
\section{Road-Network-Indistinguishability}
In this section, we propose a new definition of location privacy called road-network-indistinguishability (\rni), which tightly considers location privacy on road networks.
Firstly, We formally define privacy loss of locations on road networks caused by an output of a mechanism. Following this notion, we define privacy of the mechanism on road networks. Then, we derive the definition of $\epsilon$-\rni.
Second, we describe the characteristics of \rni\ which are inherited from $d_\mathcal{X}$-privacy~\cite{broad_dp}, which is a generalization of differential privacy.
Finally, we analyze the relationship between geo-indistinguishability and \rni.

\subsection{Privacy Loss on Road Networks}
Here, we propose a formulation of privacy loss caused by a perturbation mechanism over a road network based on the concept of differential privacy~\cite{dwork2011differential}.
The idea is that privacy loss is regarded as the degree of the distinguishability of a true location from other locations when seeing the output of a mechanism. Then, we define privacy loss on a road network as follows.
\begin{definition}[location privacy loss on a road network]
\label{def:privacyloss}
Location privacy loss on a road network of $v\in\mathcal{V}$ with respect to $v^\prime\in\mathcal{V}$ caused by $M:\mathcal{V}\to\mathcal{Z}$ is:
\begin{equation}
    L(M,v,v^\prime)=\sup_{S\subseteq{\mathcal{Z}}}|\log\frac{\Pr(M(v)\in S)}{\Pr(M(v^\prime)\in S)}|
\end{equation}
\end{definition}
Intuitively, this means that when a user at location $v$ uses mechanism $M$, an adversary can distinguish the true location $v$ from other location $v^\prime$ with the order of $L$.
The difference between ours and privacy loss of differential privacy~(Equation~\ref{equ:privacyloss}) is the domain of input and constraint of the neighboring datasets. In differential privacy, the domain is a set of dataset and neighboring datasets are defined as datasets whose only single record is different because a single record of an individual is regarded as the target to protect and the degree of its distinguishability can be regarded as the privacy. In our setting, a domain is a set of locations on road networks and any two locations corrsponds to neighboring datasets because a location is a target to protect and the degree of its distinguishability can be regarded as the privacy.

\subsection{Privacy Definition on Road Networks}
Here, we define the privacy of mechanism $M$.
As described above, privacy loss represents the degree of the distinguishability of two locations. When privacy loss caused by a mechanism is bounded by some value $l$ for any two locations, it can be said that $l$ represents the privacy protection level of the mechanism.
In other words, even if a user at location $v$ outputs a perturbed location with the mechanism, an adversary cannot distinguish the true location $v$ from other any locations $v^\prime$ in the order of $l$. This idea is formally represented as follows.
\begin{equation}
\label{equ:privacylevel}
\forall v,v^\prime\in\mathcal{V}, L(M,v,v^\prime)\leq l
\end{equation}
where $l\in\mathbb{R}^+$. Let $\mathcal{V}$ be a set of locations on road networks and $\mathcal{Z}$ be a set of outputs of a mechanism. Intuitively, if a user who is at some location uses the mechanism and outputs $z$, a true location cannot be distinguishable from all other locations on road networks to the extent of the value of $l$. If $l=0.1$, the ratio of prior probability of $v$ and posterior probability of $v$ (i.e. $\Pr(v|z)$) is up to $\mathrm{e}^{0.1}\fallingdotseq 1.1$, so an adversary cannot raise a probability that the user is at one location, which means the indistinguishability of the true location from all other locations on road networks.

Although a mechanism which satisfies Inequality~\ref{equ:privacylevel} with a small value of $l$ guarantees strong privacy protection due to the indistinguishability between any two locations, this definition restricts a mechanism too much to output a useful output.
Then, we relax the notion of neighboring locations so that neighboring locations mean the close locations from each other within the distance $r$ and we provide the indistinguishability for only the neighboring locations. Formally, we define $r$-neighboring locations as two locations such that $d_s(v,v^\prime)\leq r$ and given $\epsilon \in \mathbb{R^+}$, we define \lronroad\ as follows.
\begin{definition}[\lronroad]
\label{def:lonroad}
A mechanism $M:\mathcal{V}\to\mathcal{Z}$ satisfies \lronroad\ iff for any two $r$-neighboring locations $v,v^\prime\in\mathcal{V}$:
\begin{equation}
    L(M,v,v^\prime)\leq l
\end{equation}
\end{definition}
\lronroad\ guarantees that a true location $v$ is indistinguishable from other locations $v^\prime$ such that $d_s(v,v^\prime)\leq r$. This definition is motivated by the fact that to make two locations which are distant indistinguished causes much utility loss.
%%% end
\subsection{Road-Network-Indistinguishability}
So far, we defined privacy loss and privacy a mechanism, \lronroad. 
Here, by using these notions, we propose a formal definition of location privacy on road networks, $\epsilon$-road-network-indistinguishability (\rni).
\lronroad\ depends on two parameters $l$ and $r$. 
Intuitively, when $r$ is small, $l$ should be small because the true location needs to be protected in small range of locations.
Conversely, when $r$ is large, some distinguishability (i.e. somewhat large $l$) of a true location should be acceptable because the distinguishability in large range of locations means stronger privacy protection than in small range.
From this idea, $\epsilon$-\rni\ can be formulated as follows:
\begin{definition}[$\epsilon$-\roadi]
A mechanism $M:\mathcal{V}\to\mathcal{W}$ satisfies $\epsilon$-\roadi\ iff $\forall v,v^\prime\in\mathcal{V}$:
\begin{equation}
    L(M,v,v^\prime)\leq\epsilon d_s(v,v^\prime)
\end{equation}
where $\mathcal{W}\subseteq{\mathcal{V}}$.
\end{definition}
In other words, $\epsilon$-\rni\ guarantees the indistinguishability of the order of $\epsilon r$ between two locations such that the distance is less than $r$.
This means that for any $r\in\mathbb{R}$, $M$ satisfies $(\epsilon r, r)$-road network privacy. Intuitively, this definition allows a mechanism to linearly weaken the indistinguishability of two locations according to the distance to output a useful location, so the farther two locations are, the more distinguishable the two locations could be. We note that $\epsilon$-\rni\ requires that output range $\mathcal{W}$ is a subset of $\mathcal{V}$ for reasons described in \sect~\ref{subsec:range}. Therefore, even if a mechanism should satisfy $(\epsilon r, r)$-road network privacy for any $r$, the mechanism does not satisfy $\epsilon$-\rni\ when an output of the mechanism includes other than a location on a road network (i.e. $v\notin \mathcal{V}$).
However, any mechanism which satisfies $(\epsilon r, r)$-road network privacy for any $r$ can satisfy $\epsilon$-\rni\ by a post-processing function $f:\mathcal{Z}\to\mathcal{V}$. This is because that if $M$ satisfies \lronroad, any post-processed mechanism $f\circ M$ satisfies \lronroad\ as shown in Theorem~\ref{theo:postprocess}. 
\begin{theorem}[Post-processing theorem of \lronroad.]
\label{theo:postprocess}
If a mechanism $M:\mathcal{V}\to\mathcal{Z}$ satisfies \lronroad, a post-processed mechanism $f\circ M$ also satisfies \lronroad\ for any function $f:\mathcal{Z}\to\mathcal{Z}^\prime$.
\end{theorem}
We refer the reader to the appendix for the proof. We take Planar Laplace Mechanism~\cite{geo-i} (\plm) as an example.
The distribution of \plm\ is as follows:
\begin{equation}
        \Pr(PLM_\epsilon(x)=o) = \frac{\epsilon^2}{2\pi}\mathrm{e}^{-\epsilon d_e(x,o)}
\end{equation}
where $o\in\mathbb{R}^2$.
\plm\ satisfies $(\epsilon r, r)$-road network privacy for any $r$, but does not satisfy $\epsilon$-\rni\ because output range is not on a road network. By applying post-processing function $f:\mathcal{Z}\to\mathcal{V}$ (e.g. mapping to the nearest location on a road network), post-processed \plm\, which we call Planar Laplace Mechanism on a Graph (\plmg), satisfies $\epsilon$-\rni. 


\subsection{Output Range from Privacy Perspective}
\label{subsec:range}
There are three reasons for $\epsilon$-\rni\ to restrict output range to $\mathcal{W}\subseteq\mathcal{V}$.
First, LBSs over road networks expect to receive a location on road networks as described in \sect~\ref{subsec:problem}.

Second, \lronroad\ is not only immune to post-processing $f:\mathcal{Z}\to\mathcal{V}$ (Theorem~\ref{theo:postprocess}) but also may be enhanced by post-processing. For example, if $f$ is a function which always maps to fixed one location on road networks, this mechanism satisfies $0$-\rni. This means that post-processing always strengthen the indistinguishability. Therefore, to rigorously measure the indistinguishability of locations on road networks, the indistinguishability of a post-processed mechanism is more appropriate than the indistinguishability of the mechanism which is not post-processed.

Third, since road networks are public information, output of a location outside road networks may cause empirical privacy leaks and post-processing to a location on a road network prevents this empirical privacy leaks. We empirically show that an adversary who knows road networks can attack with higher accuracy than an adversary who does not know if a mechanism outputs a location outside a road network and a post-processed mechanism protects privacy from this attack.
To show this, we evaluate the empirical privacy gain \privacygain~(Equation~\ref{equ:privacygain}) of two kinds of mechanisms \plm\ and \plmg\ against the two kinds of adversaries. We use function $f$, which maps to the nearest location on road networks as post-processing of \plmg.

For simplicity, we use a simple synthetic map illustrated in \fig~\ref{fig:syn_map}. This map consists of 1600 squares with the side length of \SI{100}{m}; that is, the area dimensions are \SI{4000}{m} * \SI{4000}{m}, and each lattice point has a coordinate. The center line represents a road where a user is able to exist, and the other area represents locations where a user must not be, such as the sea. 
In this map, we evaluate empirical privacy gain \privacygain\ of the two mechanisms against two kinds of adversaries with same utility loss \utilityloss. We use the Euclidean distance as the metric of \privacygain\ and \utilityloss, which are denoted by \privacygain$_e$ and \utilityloss$_e$. 

\begin{figure}[t]
 \begin{minipage}{0.4\hsize}
   \centering\includegraphics[width=\hsize]{img/synthegraph.png}
  \caption{A synthetic map. The red line represents a road, and a user is located inside the black frame.}
  \label{fig:syn_map}
 \end{minipage}
\hfill
 \begin{minipage}{0.6\hsize}
   \centering\includegraphics[width=\hsize]{img/ge.eps}
  \caption{Privacy gain of each mechanism with respect to utility loss in the Euclidena distance, that is \privacygain$_e$ and \utilityloss$_e$. PLM$^*$ represents privacy gain of \plm\ against an adversary who does not know road networks.}
  \label{fig:output_outside}
 \end{minipage}
\end{figure}

\fig~\ref{fig:output_outside} shows the results. 
\plm\ represents empirical privacy gain \privacygain\ against an adversary who considers a road network and \plm$^*$ represents the one against an adversary who dose not know a road network. Comparing \plm\ with \plm$^*$, it is said that the adversary can more accurately infer the true location by considering road networks.
\privacygain\ of \plmg\ is higher than \privacygain\ of \plm\ and is almost the same as \privacygain\ of \plm$^*$. 
By restricting output to locations on a road network, adversary cannot improve the inference of the true location because additional information does not exist. In other words, post-processing to a location on road networks strengthen a empirical privacy level against an adversary who considers road networks.

In summary, a mechanism is required to output location on road networks to use LBSs over a road network, and the degree of the indistinguishability of locations brought by the post-processed mechanism is higher than the degree of the indistinguishability of a mechanism whose output range includes locations outside a road network. Moreover, from the empirical privacy point of view, a post-processed mechanism does not cause empirical privacy leaks caused by considering road networks. Therefore, $\epsilon$-\rni\ restricts output range to locations on a road network.

\subsection{Characteristics}
\rni\ is an instance of $d_\mathcal{X}$-privacy~\cite{broad_dp}, which is a generalization of differential privacy, and has following two characteristics which show strong privacy protection.

\subsubsection{Hiding function}
The first characterization uses the concept of a hiding function $\phi:\mathcal{V}\to\mathcal{V}$. For any hiding function and a secret location $v\in\mathcal{V}$, when an attacker who has a prior distribution that expresses information of user's location obtains each output $o = M(v)$ and $o^\prime = M(\phi(v))$ of a mechanism which satisfies $\epsilon$-\roadi, the following inequality holds for each posterior distribution:
\begin{equation}
\label{hiding-function}
    |\log\frac{\Pr(v|o)}{\Pr(v|o^\prime)}|\leq 2\epsilon d_s(\phi)
\end{equation}
Let $d_s(\phi(v))=sup_{v\in V}d_s(v,\phi(v))$ be the maximum distance between an actual vertex and its hidden version. This inequality guarantees that adversary's conclusions are the same (up to $2\epsilon d_s(\phi)$) regardless of whether $\phi$ has been applied or not to the secret location.
\subsubsection{Informed attacker}
\label{subsubsec:informed}
The other characterization is shown by the ratio of a prior distribution and its posterior distribution that is derived by obtaining an output of the mechanism. By measuring its value, we can determine how much the adversary has learned about the secret. We assume that an adversary (informed attacker) knows that the secret location is in $N\subseteq{\mathcal{V}}$. When the adversary obtains an output of the mechanism. The following inequality holds for the ratio of his prior distribution $\pi_{|N}(v)=\pi(v|N)$ and its posterior distribution $p_{|N}(v|o)=p(v|o,N)$:
\begin{equation}
\label{informedattacker}
    \log\frac{\pi_{|N}(v)}{p_{|N}(v|o)}\leq \epsilon d_s(N)
\end{equation}
Let $d_s(N)=max_{v,v^\prime\in N}d_s(v,v^\prime)$ be the maximum distance between locations in $N$. This inequality guarantees that when $d_s(N)$ is small, the adversary's prior distribution and its posterior distribution are similar. In other words, the more the adversary knows about the actual location, the less he cannot learn about the location from an output of the mechanism.\par


\subsection{Analyzing the Relationship between Geo-indistinguishability and Road-network-indistinguishability}
\label{subsec:analyze_relationship}
\rni\ is defined on the metric space where $d_s$ is defined, which restricts the domain to be on road networks. Here, we consider location privacy in the more general case of no constraints so that the domain is on the Euclidean plane $\mathcal{X}\subseteq{\mathbb{R}^2}$ where the Euclidean distance $d_e$ is defined. In this case, the definition is $\epsilon$-geo-indistinguishability~\cite{geo-i}.
\begin{definition}[$\epsilon$-geo-indistinguishability]
A mechanism $M:\mathcal{X}\to\mathcal{Z}$ satisfies $\epsilon$-geo-indistnguishability iff $\forall{x,x^\prime}\in\mathcal{X}$:
\begin{equation}
    \sup_{S\in{\mathcal{Z}}}|\log\frac{\Pr(M(x)\in S)}{\Pr(M(x^\prime)\in S)}|\leq\epsilon d_e(x,x^\prime)
\end{equation}
\end{definition}
Moreover, if mechanism $M:\mathcal{X}\to\mathcal{Z}$ satisfies $\epsilon$-\GeoI, following inequality holds for all two locations on road networks $v,v^\prime\in\mathcal{V}$ from Inequality~(\ref{equ:shortest-path}).
\begin{equation}
\label{equ:geo_road}
\begin{split}
    \sup_{S\in{\mathcal{Z}}}|\log\frac{\Pr(M(v)\in S)}{\Pr(M(v^\prime)\in S)}|=L(M,v,v^\prime)\leq &\epsilon d_e(v,v^\prime)\\\leq
    &\epsilon d_s(v,v^\prime)
\end{split}
\end{equation}
This derives a following theorem.
\begin{theorem}
If a mechanism $M$ satisfies $\epsilon$-\GeoI, $M$ satisfies ($\epsilon r$, $r$)-road network privacy for any $r$. Then, a post-processed mechanism $f\circ{M}$ satisfies $\epsilon$-\rni\ where $f:\mathcal{Z}\to\mathcal{V}$ is any mapping function to a location on a road network.
\end{theorem}
This is derived from Inequality~(\ref{equ:geo_road}) and post-processing theorem (Theorem~\ref{theo:postprocess}). This means that a mechanism which satisfies $\epsilon$-\GeoI\ can always convert to a mechanism which satisfies $\epsilon$-\rni\ by post-processing.
We note that the reverse is not always true. That is, \rni\ is the relaxed version of \GeoI\ by using the metric $d_s$ to output useful location for LBSs over road networks.
For example, although \plmg\ satisfies $\epsilon$-\GeoI\ and  $\epsilon$-\rni, graph-exponential mechanism (GEM) which we propose in the next section satisfies only \rni.

==> sections/optimize_backhp.tex <==
\section{Analyzing the Performance of GEM and Optimizing Range}
GEM requires output $z$ to be on a road network but require nothing else for the output range. This means that an optimal output range exists for privacy and utility.
In this section, first we apply \utilityloss\ and \privacygain\ to a location setting on road networks. Then, we propose the performance criteria (PC) which represents the tradeoff between the privacy and  the utility.
Next, we formalize an optimization problem for the PC.
Finally, we propose a greedy algorithm to solve the optimization problem in an acceptable amount of time.
%Then, we analyze the relationship between output range and \utilityloss$_s$, which is the measurement of utility loss on a road network and show what output range contributes to reduction of \utilityloss$_s$. 
%For simplicity, we assume that inputs are nodes of a graph.
%Next, we propose a method to find better output range. 
%We consider two settings where a prior distribution of a user is given (e.g., the user is near the restaurant) or not given, and we formalize an objective function for each setting. However, the computational complexity to solve this problem is not acceptable. Then, we propose an algorithm to find an approximate solution.

\subsection{Performance of a Mechanism on a Road Network}
While the $\epsilon$ of GG-I indicates the degree of indistinguishability between a real and perturbed location, it does not indicate the performance of a mechanism w.r.t its utility for some user and empirical privacy against some adversary. 
Therefore, we introduce the two notions \utilityloss$_s$\ and \privacygain$_s$ by applying \utilityloss\ and \privacygain\ (\sect~\ref{subsubsec:aeandsql}) to the setting of road networks. We provide their definitions below.

\begin{equation}
\label{equ:utilityonroad}
    \utilityloss_s(\pi_u,M) = \utilityloss(\pi_u,M, d_s) 
\end{equation}
\begin{equation}
\label{equ:privacygainonroad}
    \privacygain_s(\pi_a,M,h) = \privacygain(\pi_a, M, h, d_s)
\end{equation}

Intuitively, SQL$_s$\ is the expected distance on road networks between the true locations and perturbed locations, while AE$_s$\ is the expected distance on road networks between the true locations and the locations inferred by an adversary. 
In the following, we let SQL and AE denote SQL$_s$\ and AE$_s$.
We note that, as opposed to $\epsilon$, \privacygain\ changes according to the assumed adversary (i.e., the specific attack method and prior distribution). 
However, because AE increases as SQL increases (e.g., a mechanism that outputs a distant location will result in high AE but also high SQL), using only AE as a performance criterion for a mechanism is not appropriate.
Then, we define a new criterion to measure the performance of a mechanism against an assumed adversary, which we call the performance criterion (PC).

\begin{equation}
    PC=AE/SQL
\end{equation}
Intuitively, against an assumed adversary, PC represents the size of AE with respect to the SQL. In other words, PC measures the utility/privacy tradeoff.
For example, if an adversary with an optimal attack~\cite{shokri-strategy} cannot infer the true location at all (i.e., the adversary infers the pseudolocation as the true location), the mechanism can be considered as having the highest performance ($PC=1$). Conversely, the mechanism performs worst ($PC=0$) if the adversary can always infer the true location.



\subsection{Objective Functions}
%Here, we propose two objective functions to find the optimal output range of \gem\ according to two settings where some prior knowledge (i.e., a prior distribution of a user) is not given and given.


\subsubsection{An Objective Function for Utility}
When prior knowledge is not given, we cannot compute \utilityloss\ and \privacygain. However, by assuming some prior distribution of a user, \utilityloss\ can be computed. Then, the objective function for utility can be formalized as follows.
\begin{mini}|l|
{\mathcal{W}\subseteq{V}}{\utilityloss_{\mathcal{W}}}{}{}
\end{mini}
If a user does not follow the assumed distribution, the solution of \utilityloss\ may not be optimal. However, for example, \utilityloss\ for the uniform distribution represents the average of utility loss of each input (i.e., \eachutilityloss) and the optimal mechanism for the uniform distribution will not result in bad utility for any input. Therefore, this optimization is worth to do even if the prior knowledge is not given.

\subsubsection{An Objective Function for Empirical Privacy}
\label{subsubsec:obj_fn_for_empirical_privacy}
Here, we consider a setting where prior knowledge is given. The example of the setting where prior knowledge is given is shown in \sect~\ref{subsubsec:scenario}. We can compute \privacygain\ in this setting by assuming some inference function (we refer to \sect~\ref{subsubsec:userandadv} for detail). We use a posterior distribution given perturbed location $o$ as inference function $h$ because this inference is general. 
%By assuming such adversary, the solution will not result in a bad privacy level for any adversary.
The posterior distribution is as follows from Bayesian theorem.

\begin{equation}
\label{equ:post}
    h(v) = p(v|o)=\frac{p(v)p(o|v)}{p(o)}
\end{equation}

\begin{equation}
    p(o)=\sum_{v\in{\mathcal{W}}}\pi_a(v)\Pr(\gem_\mathcal{W}(v)=o)
\end{equation}

\begin{equation}
    p(v)p(o|v)=\pi_a(v)\Pr(\gem_\mathcal{W}(v)=o)
\end{equation}
\mc$_\mathcal{W}$ can be formulated as follows by using posterior distribution as the inference function.

\begin{equation}
    \frac{\sum_{v,\hat{v}\in\mathcal{V},o\in\mathcal{W}}\pi_u(v)\Pr(\gem_\mathcal{W}(v)=o)p(\hat{v}|o)d_s(v,\hat{v})}{\sum_{v\in\mathcal{V},o\in\mathcal{W}}\pi_u(v)\Pr(\gem_\mathcal{W}(v)=o)d_s(v,o)}
\end{equation}
Then, the objective function against the adversary can be formulated as follows.
\begin{maxi}|l|
{\mathcal{W}\subseteq{V}}{\mc_{\mathcal{W}}}{}{}
\end{maxi}
\gem\ with the optimized output range is considered to show the best utility-privacy trade-off against the adversary, but it can be not useful (i.e. large \utilityloss) because \utilityloss\ has no constraints, so we add the constraints to \utilityloss.

\begin{maxi}|l|
{\mathcal{W}\subseteq{V}}{\mc_\mathcal{W}}{}{}
\addConstraint{\utilityloss_{\mathcal{W}} \leq \theta}
\end{maxi}

The optimal \gem\ shows the best utility-privacy trade-off in \gem\ with an output range which shows the better \utilityloss\ than $\theta$.


\subsection{Algorithm to Find an Approximate Solution}
\label{subsec:tactic}
Since the number of combinations of the output range is $2^{|V|}$, it is difficult to find optimal solutions for these optimization problems in acceptable time, so we use a simple algorithm to find approximate solutions. We show a pseudocode of this algorithm in Algorithm~\ref{alg:opt}. The constraint function is a function which returns whether the constraint holds or does not hold.


\begin{algorithm}             
\caption{Finding a local solution.}         
\label{alg:opt}                          
\begin{algorithmic}[1]
\REQUIRE {Privacy parameter $\epsilon$, graph $G=(V,E)$ objective function $f$, constraint function $c$.}
\ENSURE {Output range $\mathcal{W}$.}
\STATE $\mathcal{W} \Leftarrow V$ 
\WHILE{True}
\STATE $\mathcal{W}_0 \Leftarrow \mathcal{W}$
\STATE $obj \Leftarrow f(GEM_{\mathcal{W}_o})$

\FOR{$v$ in $V$}
\STATE $\mathcal{W}^\prime \Leftarrow \mathcal{W}\setminus \{v\}$
\STATE $obj^\prime \Leftarrow f(GEM_{\mathcal{W}^\prime})$
\STATE $cons \Leftarrow c(GEM_{\mathcal{W}^\prime})$
\IF{$obj^\prime - obj < 0$ and cons}
\STATE $\mathcal{W} \Leftarrow W^\prime$
\STATE $obj \Leftarrow obj^\prime$
\ENDIF
\ENDFOR
\IF{$\mathcal{W}_0 = \mathcal{W}$}
\STATE break
\ENDIF
\ENDWHILE
\STATE return $\mathcal{W}$
\end{algorithmic}
\end{algorithm}

First, we start with an output range which includes all nodes (i.e., $V$). Next, we compute a value of the objective function of the output range whose one node is removed. We remove the node if the objective function improves and the constraint holds, and we repeat until it converges. We repeat this procedure until convergence of the objective function. This computational complexity is $O(|V|^2)$ when the computational complexity of the objective function is $O(1)$. As a rule of thumb, the main loop (line 2 of Algorithm \ref{alg:opt}) likely finish in the small number of iterations.
However, the computational complexities of \utilityloss\ and \mc\ are $O(|V|^2)$ and $O(|V|^3)$, so the overall computational complexities are $O(|V|^4)$ and $O(|V|^5)$. In the following, we approximate the objective functions so that the computational complexities are acceptable.

\subsubsection{Approximation of SQL}
We approximate \utilityloss\ using an approximation of \eachutilityloss\ as follows.
\begin{equation}
\label{equ:sql_approx}
\begin{split}
    SQL_{\mathcal{W}} &= \sum_{v\in V}\pi_u(v)\hat{SQL}_\mathcal{W}(v)\\ &\approx \sum_{v\in V}\pi_u(v)\sum_{v^\prime\in A_k(v)} \Pr(\gem_{A_k}(v) = v^\prime)d_s(v,v^\prime) 
\end{split}
\end{equation}
where $A_k(v)$ is the set of nodes which are the top $k$ nearest nodes in $\mathcal{W}$ from $v$. \gem\ rarely outputs a distant location from an input, so we assume that the affect of the output to \utilityloss\ can be negligible. From this fact, we use only the $k$ nearest nodes for computing \utilityloss. 
In this paper, we use $k$ as $50$.
This computational complexity is $O(k|V|)$. 
Then, the computational complexity of Algorithm \ref{alg:opt} is $O(k|V|^3)$.
We note that if nodes are uniformly distributed, the removal of one node $v_r$ affects $k$ nodes of $\hat{SQL}_\mathcal$, so the computational complexity of \utilityloss$_{\mathcal{W}\setminus\{v_r\}}$ is $O(k^2)$. We show the example the case of $k=10$ in \fig~\ref{fig:opt}.
In this case, the computational complexity of Algorithm \ref{alg:opt} is $O(k^2|V|^2)$.

\subsubsection{Approximation of \mc}
We approximate \mc\ using an approximation of \utilityloss\ (i.e., Equation~\ref{equ:sql_approx}) and \privacygain\ in the same way as follows.

\begin{equation}
\label{equ:ae_approx}
\begin{split}
&\privacygain \approx\\ &\sum_{v\in\mathcal{W}}\pi_u(v)\sum_{\hat{v},v^\prime\in A_k(v)}\Pr(GEM_{A_k(v)}(v)=v^\prime)\Pr(\hat{v}|v^\prime)d_s(\hat{v},v)
\end{split}
\end{equation}
The posterior distribution (Equation~\ref{equ:post}) can be computed in $O(k^2)$ when \gem$_{A_k(v)}$ is used. Then, this computational complexity of \privacygain\ is $O(k^2|V|)$, so the computational complexity of Algorithm \ref{alg:opt} is $O(k^2|V|^3)$.
\mc\ is computed from \privacygain\ and \utilityloss, the computational complexity of \mc\ is $O(k^2|V|)$. 
As the case of \utilityloss, if nodes are uniformly distributed, \privacygain\ can be computed in $O(k^3)$.
In that case, the computational complexity of Algorithm \ref{fig:opt} is $O(k^3|V|^2)$.


\subsection{Examples of Optimizations}

\begin{figure}[t]
 \begin{minipage}{0.5\hsize}
   \centering\includegraphics[width=\hsize]{img/prior_unbr_synth.png}
  \caption{Synthetic map whose side length is \SI{1500}{m}. Axis represents the prior probability.}
  \label{fig:synth_unbr_map}
 \end{minipage}
\hfill
 \begin{minipage}{0.5\hsize}
  \begin{minipage}{\hsize}
   \centering\includegraphics[width=0.5\hsize,height=0.5\hsize]{img/synth_opt_sql.png}
  \end{minipage}
  \begin{minipage}{\hsize}
   \centering\includegraphics[width=0.5\hsize,height=0.5\hsize]{img/synth_opt_mc.png}
  \end{minipage}
   \caption{Each solution for \utilityloss\ (above) and \mc\ (below). The blue points represent node to output.}
   \label{fig:solutions_synth}
 \end{minipage}
 \begin{minipage}{0.5\hsize}
   \centering\includegraphics[width=\hsize]{img/time.eps}
  \caption{The relationship between the number of nodes and time required for the optimization.}
  \label{fig:time}
 \end{minipage}
 \begin{minipage}{0.5\hsize}
   \centering\includegraphics[width=\hsize]{img/opt.png}
  \caption{An example of affected nodes by a removed node when $k=10$.}
  \label{fig:opt}
 \end{minipage}
\end{figure}

Here, we show the example of the optimization in the synthetic map. First, we explore the relationship between the number of nodes and the time required for the optimization. We use several lattices whose number of nodes are different (\fig~\ref{fig:square_graphs}). We use Python 3.7, OS Ubuntu 15.10 and CPU Intel core i7 6770k and memory of 64GB as the computational environment.
We show the results in \fig~\ref{fig:time}.
We can see that even if the node size is large (e.g., $>10000$), the algorithm finishes within $1$ hour.
This is acceptable because we can run this algorithm for future perturbation in advance.
We note that it takes more time for the optimization w.r.t \utilityloss\ than that of \mc\ despite of the larger computational complexity of \mc. This is because, in my experience, main loop (line 2 of Algorithm~\ref{alg:opt}) finishes in the smaller iterations for the optimization of \mc. As the examples of the number of nodes, graphs in \fig~\ref{fig:maps} whose ranges are \SI{1000}{m} from the center have $1155$ and $168$ nodes. Even if a graph is quite large, by separating to the small graphs such as \fig~\ref{fig:maps}, we can run the algorithm in the acceptable time.


Next, we ran the algorithm using the synthetic map (\fig~\ref{fig:synth_unbr_map}) under the assumption of the prior distribution. We assume that there are four places where the prior probability is high as shown in \fig~\ref{fig:synth_unbr_map} and a user who follows this prior probability uses \gem\ with $\epsilon=0.01$ and an adversary has knowledge of this prior distribution. In this case, \utilityloss\ is \SI{328}{m} and \mc\ is $0.9$.
First, a solution for utility (i.e., objective function (23)) is as the upper side of~\fig~\ref{fig:solutions_synth}. By restricting output in the place where the prior probability is high, lower utility loss ($\utilityloss =\SI{290}{m}$) can be achieved. Next, a solution for \mc\ (i.e., objective function (28)) is as the lower side of~\fig~\ref{fig:solutions_synth}. It can be seen that output range is more restricted to the place with the high prior probability than the case of the solution for utility. This causes utility loss ($\utilityloss=\SI{301}{m}$), but higher \mc\ is achieved ($\mc =1.0$) than the solution for \utilityloss\ where $\mc = 0.98$. The adversary cannot but believe the pseudolocation is the true location, which means that the mechanism can effectively perturb the true location.
